Impact of correlations on topology in Kane-Mele model decorated with impurities

We propose an effective model for the study of the interplay between correlation and topology by decorating the Kane-Mele model with a set of localized interacting orbitals hybridized to just one sublattice, breaking the inversion symmetry. We show that in the time-reversal symmetric case, the interplay between interactions and hybridization extends the stability of the topological phase and depending on the driving mechanism very different behaviors are observed after the topological phase transition (TPT). We discuss the fate of the TPT in presence of weak ferromagnetic order, by introducing a weak local magnetic field at the localized orbitals, which splits the two band inversion points. One of the platforms to apply this model to are ferrovalley compounds, which are characterized by two independent band inversion points. Understanding this family of materials is crucial for the development of the valleytronics. An alternative to spintronics, which uses valley polarization as opposed to spin degrees of freedom as the building block, promises great opportunities for the development of information storage.

==> appedix.tex <==
\begin{document}


\section{Limit cases}
Before discussing the results of the full model it is helpful to look at the solution of two limiting cases: the non-interacting localized orbitals $U$=0, and the isolated cluster (bottom panel of Fig. \ref{lattice:fig}).

In the first case for $U$=0, the model is exactly solvable, and it can give a rough idea about the fate of the topology of the QSH system in the presence of hybridization with additional, inversion symmetry breaking, localized states. From the point of view of the topology the gaps at $K$ and $K^\prime$ are crucial, since that is where the non-zero Berry curvature originates. At these points the non-interacting Hamiltonian in the spin-up channel and in the basis of $\{$sublattice A, sublattice B, localized orbitals$\}$ at $K/K^\prime$ point is given by 
\begin{equation}
\mathcal{H}(\vec{k}=K)=\left[
    \begin{array}{ccc}
         \alpha & 0  & 0\\
         0 & -\alpha & J\\
         0 & J & \delta
    \end{array}
    \right]
\end{equation}
,where sign of $\alpha=\pm 3\sqrt{3}t^\prime$ depends on the valley ($K$ or $K^\prime$ point) and $\delta$ is the localized orbital level. This Hamiltonian has one orbital detached from the other two hence its energy level $E_0$ is unaltered by $J$. The remaining two states form an admixture of the lattice and localized orbitals resulting in 
\begin{equation}
\begin{array}{c}
     E_0=\alpha,\\
     E_\pm=\frac{\delta -\alpha}{2} \pm \sqrt{J^2+\left(\frac{\delta +\alpha}{2}\right)^2} .
\end{array}
\end{equation}
Due to the hybridization, the $E_-$ and $E_+$ energy levels repel each other with strength that depends on the relative position of these two orbitals' energy levels. Because one level is unchanged and two other levels repel, increasing $J$ will eventually lead to the closing of the gap between $E_0$ and one of the $E_-, E_+$ states.
The presence of an additional state means that the topological gap for the non-interacting model is not at half-filling, as in the standard KMM, but for either $\frac{1}{3}$ or $\frac{2}{3}$ fillings. 
In the following sections we will focus on the $\frac{2}{3}$ filling case and only mention the $\frac{1}{3}$ filling if it is different from the former. 
In the non-trivial topological phase, $\alpha$ changes sign as one goes along the $K\rightarrow K^\prime$ path and the unaltered energy level shifts from the above to below the hybridized pair of states. Thus as $J$ grows the initially flat band of the localized electrons, located somewhere in the KMM gap, will start to gain a substantial amount of dispersion as the band bending will be in opposite directions at either valley. Introducing an additional sub-lattice splitting mass term, which turns the underlying KMM into a BI, makes the sign of the gap positive along the $K-K^\prime$ path. In this case, switching on the hybridization term will result in a much less dispersive band, as the unaltered state is always above/below the hybridized ones. Nonetheless, sufficiently strong  $J$ will lead to band inversion.
%\textbf{WB: what is the AZ symmetry class and invariant of the non-interacting model? Was it calculated? JS: No clue about the symmetry class to be honest. I was never smart enough to understand the ins and outs of Zirnbauers paper on the periodic table of TIs}

\begin{figure}
\flushleft
\includegraphics[width=0.48\textwidth]{doped_G0_J_dep.pdf}
\includegraphics[width=0.48\textwidth]{doped_G0_U_dep.pdf}
\caption{Evolution of the spectral function of an isolated cluster as a function of hybridization strength $J$ top panel, and interaction strength $U$. In the top panel $U=0.5$ and in the bottom panel $J=0.6$. Color gradient represents the logarithm of the intensity of the peaks in the spectral function.}
\label{G0s:fig}
\end{figure}

The second limit case is the isolated cluster Greens function (depicted in the bottom panel of Fig. \ref{lattice:fig}). The isolated cluster Greens function $\mathcal{G}_0(\omega)$ plays a central role in the CPT approach, as it holds all the information about local charge dynamics. The information encapsulated in $\mathcal{G}_0(\omega)$ is especially important for the model studied in this work. The reduction in the dimensionality of the cluster coupling matrix from a 3x3, in a general case, to  2x2 results in the equality between the localized orbital part of the diagonal part of the Greens function of the full lattice and the isolated cluster. Thus it is useful to analyze properties of $\mathcal{G}_0(\omega)$ before going into details of the Greens function for the whole system.
In the Fig. \ref{G0s:fig} the evolution of the spectra of $\mathcal{G}_0(\omega)$ of the three-site cluster describing the unit cell is shown as a function of $J$ for a weakly interacting case (top panel) and as a function of $U$ for weak hybridization (bottom panel). In both panels, the black dashed lines indicate the position of the peaks in the corresponding non-interacting model as a reference point. The position of these lines and the peaks of $\mathcal{G}_0(\omega)$ with the most spectral weight follow each other closely, highlighting a connection between the $\frac{2}{3}$ filled case and the single-particle picture. The biggest discrepancy between the two can be seen in the position of the middle peak.
A comparison between the $U$-evolution and $J$-evolution of this peak shows, that it approaches the single particle level as $J$ is increased, but deviates from it almost linearly with $U$. This indicates the fact that at $U/J \ll 1$ the excitation spectrum has a strong orbital mixing typical for the non-interacting limit, whereas for $U/J \gg 1$ the orbital nature is recovered. In this limit the spectrum of the central correlated orbital approaches that of a fully occupied single-site Hubbard model, hence the $U$ dependence.
In either limit, the presence of the other, relatively much smaller, parameter is not negligible. In general, the complete spectrum of $\frac{2}{3}$ filled $\mathcal{G}_0(\omega)$ consists of the middle peak, described above, and three pairs of peaks placed symmetrically around a certain energy. In the $J/U \ll 1$ limit this energy is the middle peak energy, cf. top panel of Fig. \ref{G0s:fig}.
Simultaneous action of interactions and hybridization brings additional splitting of all of the bottom peaks from these three pairs. It stems from the doping away from half-filling, which breaks the particle-hole symmetry.

%electron-like
The electron-like excitation spectrum belongs to the 5/6 filling subspace of the Hilbert space. In a simplified picture, the lowest peak in $\mathcal{G}_0(\omega)$ corresponds to all sites being doubly occupied except for the one with the Hubbard term. Hence, it follows the non-interacting limit result, the dashed line in Fig. \ref{G0s:fig}. The other two have this site doubly occupied and differ in the occupancy of the non-interacting sites. Through hopping term, these two states mix resulting in additional splitting of the energy levels. This simplified picture becomes almost exact in the limit of $U/J \ll 1$, where the eigenbasis and orbital basis start to match and as a result, the splitting of the two highest energy levels approaches the value of $2$. %TODO: NOT EXACTLY CONVINCED WITH MY THINKING
%hole
The hole-like part of the excitation spectrum of the cluster resides in the 1/2 filling subspace of the Hilbert space of the cluster. It can be divided into two groups of states: with and without a doubly occupied site. The latter has a similar structure to the 5/6 filling subspace, thus mirroring its energy. The presence of the former states allows for additional splitting of these energy levels through additional charge delocalization. Which can result in kinetic energy grain/loss depending on the admixture of orbital centered around the interacting site. 


\end{document}
